LiDAR-NeRF: Novel LiDAR View Synthesis via Neural Radiance Fields

We introduce a new task, novel view synthesis for LiDAR sensors. While traditional model-based LiDAR simulators with style-transfer neural networks can be applied to render novel views, they fall short of producing accurate and realistic LiDAR patterns because the renderers rely on explicit 3D reconstruction and exploit game engines, that ignore important attributes of LiDAR points. We address this challenge by formulating, to the best of our knowledge, the first differentiable end-to-end LiDAR rendering framework, LiDAR-NeRF, leveraging a neural radiance field (NeRF) to facilitate the joint learning of geometry and the attributes of 3D points. However, simply employing NeRF cannot achieve satisfactory results, as it only focuses on learning individual pixels while ignoring local information, especially at low texture areas, resulting in poor geometry. To this end, we have taken steps to address this issue by introducing a structural regularization method to preserve local structural details. To evaluate the effectiveness of our approach, we establish an object-centric multi-view LiDAR dataset, dubbed NeRF-MVL. It contains observations of objects from 9 categories seen from 360-degree viewpoints captured with multiple LiDAR sensors. Our extensive experiments on the scene-level KITTI-360 dataset, and on our object-level NeRF-MVL show that our LiDAR-NeRF surpasses the model-based algorithms significantly.

==> latex/fig/dataset_all.tex <==
% \begin{figure*}[ht]
% 	\centering
%     \includegraphics[width=0.95\textwidth]{imgs/dataset.png}
%     % \vspace{-0.4cm}
%     \caption{\textbf{\name dataset.}}
% 	\label{fig:dataset}
% 	\vspace{-6pt}
% \end{figure*}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{imgs/dataset2.pdf}
    % \vspace{-0.4cm}
    \caption{\textbf{Dataset visualization.} Our \datasetname{} dataset encompasses 9 objects from common traffic categories. We align multiple frames here for better visualization.}
    \label{fig:dataset}
    \vspace{-2pt}
\end{figure}


==> latex/fig/edit.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{imgs/edit7.pdf}
    % \caption{\textbf{Scene editing.}
    % The top-middle portion first introduces the \textcolor{cyan}{blue} background point clouds and the \textcolor{yellow}{yellow} object point clouds, e.g., the car.
    % Dashed rectangles show the promising results of novel scene arrangements through combining the object-level output of our \name{} in various novel viewpoints. Best viewed in color and zoom in for details. \MS{I do not understand the figure, so I cannot really revise the caption.}}
    \caption{\textbf{Scene editing.}
        % One natural application of our framework is to perform scene editing.
        We augment an original scene~(top) by placing an object at an arbitrary point and in an arbitrary pose. Note that the augmented scene~(bottom) has realistic occlusion effects thanks to our pseudo range-image formalism. Best viewed in color and zoomed in.
        See the supplementary material for more visual examples.
        % \tao{The top portion is the
        % Dashed rectangles show the promising results of novel scene arrangements through combining the object-level output of our \name{} in various novel viewpoints. Best viewed in color and zoom in for details. }
    }

    \label{fig:scene-edit}
    \vspace{-4pt}
\end{figure}


==> latex/fig/lidarnerf.tex <==
\begin{figure}[t]
    \begin{center}
        \includegraphics[width=1\linewidth]{imgs/lidar-nerf6.pdf}
    \end{center}
    \vspace{-4pt}
    \caption{\textbf{Our \name{} framework.} Taking multi-view
        %rays of
        LiDAR range images with associated sensor poses as input, our model produces 3D representations of the distance, the intensity and the ray-drop probability at each pseudo pixel. We exploit multi-view consistency of the 3D scene to help our network produce accurate geometry.}
    \label{fig:LiDAR-NeRF}
    \vspace{-4pt}
\end{figure}


==> latex/fig/mesh.tex <==
\begin{figure*}[ht]
    \centering
    \vspace{-0.3cm}
    \includegraphics[width=0.7\linewidth]{imgs/mesh.png}
    \caption{\textbf{The explicit reconstruction of baseline simulators.} The explicit 3D mesh reconstruction of LiDAR point clouds suffers from inaccuracy and tends
        to overestimate the object surface.
    }
    \label{fig:mesh}
\end{figure*}


==> latex/fig/rangeview.tex <==
% \begin{figure}[t]
% \begin{center}
%   \includegraphics[width=1\linewidth]{imgs/rangeview4.pdf}
% \end{center}
%   \vspace{-8pt}
%    \caption{\textbf{LiDAR model and range image representation.}
%    \textbf{(Top)} The physical model of a LiDAR can be described as follow. Each laser beam originates from the sensor origin and shoot outwards to a point in the real world or vanishes. One common pattern of laser beam is spinning in a 360-degree fashion. \textbf{(Bottom)} We convert the point clouds into a range image, where each pixel corresponds to a laser beam. Note that we highlight one object in the different views to facilitate the visualization.
%    % The LiDAR sensor uses spinning laser beams to create a 3D model of the environment, which can be represented as a point cloud. The point cloud can be converted to a range image, where each pixel corresponds to a point in the 3D model. We highlight the same tree in different views and representations for better illustration.
%    % \tao{color}
%    }
% \label{fig:rangeview}
%   \vspace{-4pt}
% \end{figure}



\begin{wrapfigure}{r}{6.9cm}
    \vspace{-30pt}
    \includegraphics[width=\linewidth]{{imgs/rangeview4.pdf}}
    % \captionsetup{font={small}}
    % \captionsetup{width=0.9\linewidth}
    \caption{\textbf{LiDAR model and range image representation.}
        \textbf{(Top)} The physical model of a LiDAR can be described as follow. Each laser beam originates from the sensor origin and shoots outwards to a point in the real world or vanish. One common pattern of laser beams is spinning in a 360-degree fashion. \textbf{(Bottom)} We convert the point clouds into a range image, where each pixel corresponds to a laser beam. Note that we highlight one object in the different views to facilitate the visualization.
        % The LiDAR sensor uses spinning laser beams to create a 3D model of the environment, which can be represented as a point cloud. The point cloud can be converted to a range image, where each pixel corresponds to a point in the 3D model. We highlight the same tree in different views and representations for better illustration.
        % \tao{color}
    }
    \vspace{-8pt}
    \label{fig:rangeview}
\end{wrapfigure}


==> latex/fig/raydrop.tex <==
\begin{figure}[ht]
    \begin{center}
        \includegraphics[width=0.95\textwidth]{imgs/raydrop.png}
    \end{center}
    \caption{Raydrop.}
    \label{fig:Raydrop}
\end{figure}


==> latex/fig/square.tex <==
\begin{figure}[ht]
    \begin{center}
        \includegraphics[width=0.85\linewidth]{imgs/path.pdf}
    \end{center}
    % \vspace{-2pt}
    \caption{\textbf{Drive planning and sensor placements.}}
    \label{fig:square_path}
\end{figure}


==> latex/table/ablation_patch.tex <==
\begin{table*}[ht]
    % \footnotesize\centering\addtolength{\tabcolsep}{1.1pt}
     % \vspace{-0.2cm}
     \centering
     % \addtolength{\tabcolsep}{0.1pt}
     %  \begin{tabularx}{0.95\textwidth}{l|cccccccccc}
     \caption{\textbf{Ablations of our \name{}.  * donates alternating patch-wise training and pixel-wise training. }}
\vspace{-0.2cm}
         \addtolength{\tabcolsep}{0.8pt}
         \resizebox{1\textwidth}{!}{
      \begin{tabularx}{1\textwidth}{l|cccccccc}
        \toprule
 Component & C-D$\downarrow$  & F-score$\uparrow$    & RMSE$\downarrow$ & $\delta$1$\uparrow$ & $\delta$2$\uparrow$       & $\delta$3$\uparrow$  &  SSIM$\downarrow$ & MAE$\downarrow$\\
\midrule 

\midrule 
 64 x 64 & 0.0790 & 92.92 & 3.646 & 79.64 & 80.72 & 81.17 & 15.91 & 0.188 \\
 32 x 32 \\
 16 x 16 \\
 8 x 8 \\
 % 8x8 & 0.0772 & 93.03 &  3.58768815 & 0.81396367 & 0.82496322 & 0.82923286 16.27 & 0.238 \\
 8 x 8* & 0.0783 & 93.15 & 3.520 &81.81 & 82.87 & 83.30 & 16.32 & 0.243 \\
 1x1 & \\
\bottomrule
      \end{tabularx}
      }
     \label{tab:ablation_patch}
     \vspace{-4pt}
   \end{table*}

   

==> latex/table/datasets.tex <==
% \vspace{-6pt}
\begin{table*}[ht]
    % \footnotesize\centering
    % \addtolength{\tabcolsep}{-1pt}
     % \vspace{-0.2cm}
     \centering
      \begin{tabularx}{0.97\textwidth}{ll|cccc}
        \toprule
        Dataset & Component & C-D$\downarrow$  & F-score$\uparrow$    & RMSE$\downarrow$ & $\delta$1$\uparrow$ & $\delta$2$\uparrow$       & $\delta$3$\uparrow$  & PSNR$\uparrow$ & SSIM$\uparrow$\\
			\midrule 

\midrule 



			\bottomrule
      \end{tabularx}
\vspace{8pt}
\caption{\textbf{Datasets }.}
     \label{tab:exp_kitti}
   \end{table*}
   

==> latex/table/kitti_exp.tex <==
\begin{table*}[t]
  \centering
  \caption{\textbf{Novel LiDAR view synthesis on KITTI-360}. \name{} outperforms the baseline in all metrics.
    \KY{We should not list NeRF, InstantNGP as baseline. They are not. We are first to do LiDAR-NeRF, they belong to ablation study.
      Instead, consider: 1) LiDAR-NeRF (with NeRF), 2)LiDAR-NeRF (with InstantNGP), 3) LiDAR-NeRF (NeRF) + Local loss, 4) LN-NGP + Local loss.
    }
  }% by a comfortable margin.}
  \vspace{-0.2cm}
  \resizebox{1\textwidth}{!}{
    % \addtolength{\tabcolsep}{-2pt}
    \begin{tabularx}{1\textwidth}{l|cccccccc}
      \toprule
      Method                   & C-D$\downarrow$ & F-score$\uparrow$ & RMSE$\downarrow$ & $\delta$1$\uparrow$ & $\delta$2$\uparrow$ & $\delta$3$\uparrow$ & SSIM$\uparrow$ & MAE$\downarrow$ \\
      \midrule
      LiDARsim~\cite{manivasagam2020lidarsim}                                                                                                                                                \\
      PCGen~\cite{li2022pcgen} & 0.220           & 87.75             & 4.029            & 77.35               & 79.95               & 81.05               & 0.220          & 0.238           \\

      \midrule
      \textbf{\name{}}         & \textbf{0.077}  & \textbf{92.98}    & \textbf{3.511}   & \textbf{82.25}      & \textbf{83.28}      & \textbf{83.73}      & \textbf{0.365} & \textbf{0.096}  \\


      % \midrule
      % \multicolumn{3}{l}{\textit{\textbf{\name{}}}}\\
      % \midrule
      % w NeRF~\cite{mildenhall2021nerf} &  0.126 & 87.64 &3.948 & 78.26& 79.57& 80.09& 0.257 & 0.226  \\
      % w iNGP~\cite{muller2022instantNGP} &0.088 & 92.00 & 3.577 & 80.40 & 81.47 & 81.87 & 0.342 & 0.101\\
      % % d1i1
      % % d1e1i1e1 ing
      % % d1e2i1 x
      % % d1e2i1e1

      % \textbf{w iNGP \& StrucReg} & \textbf{0.077} & \textbf{92.98} & \textbf{3.511} &  \textbf{82.25} & \textbf{83.28} & \textbf{83.73} & \textbf{0.365} & \textbf{0.096}\\


      \bottomrule
    \end{tabularx}
  }
  \label{tab:exp_kitti}
\end{table*}
%  \vspace{-6pt}

%


==> latex/table/selfdata_exp1.tex <==
\begin{table*}[h!]
  % \footnotesize\centering\addtolength{\tabcolsep}{1.1pt}
  % \vspace{-0.2cm}
  \centering
  % \addtolength{\tabcolsep}{0.1pt}
  %  \begin{tabularx}{0.95\textwidth}{l|cccccccccc}
  \caption{\textbf{Novel LiDAR view synthesis on \datasetname{}}. Our \name{} outperforms the baseline in all metrics.
    %The Chamfer Distance~(C-D) in which it doesn't are biased by the density of the point clouds generated by the baseline. See \cref{fig:self-data-res} for a visual example.
    % And we find that the better C-D and F-score of the baseline are due to the fact that it generates overly dense point clouds.
  }
  \vspace{-0.2cm}
  \addtolength{\tabcolsep}{0.8pt}
  \resizebox{1\textwidth}{!}{
    \begin{tabularx}{1\textwidth}{l|cccccccc}
      \toprule
      Object-Category & C-D$\downarrow$ & F-score$\uparrow$ & RMSE$\downarrow$ & $\delta$1$\uparrow$ & $\delta$2$\uparrow$ & $\delta$3$\uparrow$ & SSIM$\uparrow$ & MAE$\downarrow$ \\
      \midrule \midrule
      \multicolumn{3}{l}{\textit{\textbf{LiDARsim~\cite{manivasagam2020lidarsim} }}}                                                                                                \\
      \midrule
      Bollard         & 0.011           & 98.92             & 5.751            & 84.64               & 84.64               & 84.64               & 0.518          & 2.172           \\
      Car             & 0.067           & 94.06             & 6.331            & 82.35               & 82.37               & 82.37               & 0.645          & 1.426           \\
      Pedestrian      & 0.011           & 97.91             & 4.788            & 90.20               & 90.20               & 90.20               & 0.748          & 4.353           \\
      Pier            & 0.016           & 95.33             & 6.606            & 78.67               & 78.67               & 78.67               & 0.510          & 2.541           \\
      Plant           & 0.018           & 93.81             & 5.315            & 86.45               & 86.45               & 86.45               & 0.667          & 0.852           \\
      Safety barrier  & 0.015           & 97.95             & 6.697            & 78.29               & 78.29               & 78.29               & 0.565          & 5.801           \\
      Tire            & 0.021           & 95.45             & 6.936            & 75.53               & 75.53               & 75.53               & 0.566          & 0.457           \\
      Traffic cone    & 0.013           & 99.59             & 5.861            & 88.14               & 88.14               & 88.14               & 0.628          & 19.14           \\
      Warning sign    & 0.024           & 91.05             & 5.569            & 86.57               & 86.57               & 86.57               & 0.663          & 0.546           \\
      \midrule
      Average         & 0.022           & 96.01             & 5.984            & 83.43               & 83.43               & 83.43               & 0.612          & 4.143           \\

      \midrule \midrule
      \multicolumn{3}{l}{\textit{\textbf{PCGen~\cite{li2022pcgen}}}}                                                                                                                \\
      \midrule

      Bollard         & 0.021           & 96.71             & 9.928            & 57.43               & 57.43               & 57.43               & 0.082          & 4.046           \\
      Car             & 0.446           & 72.23             & 5.829            & 86.37               & 86.37               & 86.37               & 0.331          & 0.123           \\
      Pedestrian      & 0.063           & 92.43             & 4.364            & 92.61               & 92.61               & 92.61               & 0.472          & 6.073           \\
      Pier            & 0.017           & 96.92             & 9.534            & 58.11               & 58.11               & 58.11               & 0.088          & 4.557           \\
      Plant           & 0.021           & 91.33             & 6.729            & 76.26               & 76.26               & 76.26               & 0.280          & 1.475           \\
      Safety barrier  & 0.070           & 74.88             & 5.382            & 87.33               & 87.33               & 87.33               & 0.207          & 5.689           \\
      Tire            & 0.026           & 94.84             & 8.748            & 62.58               & 62.58               & 62.58               & 0.095          & 0.714           \\
      Traffic cone    & 0.014           & 98.52             & 8.698            & 71.80               & 71.80               & 71.80               & 0.223          & 32.26           \\
      Warning sign    & 0.020           & 95.77             & 8.810            & 65.72               & 65.72               & 65.72               & 0.171          & 1.472           \\
      \midrule
      Average         & 0.078           & 90.40             & 7.558            & 73.13               & 73.13               & 73.13               & 0.217          & 6.268           \\


      \midrule \midrule
      \multicolumn{3}{l}{\textit{\textbf{\name{} (w/ NeRF)}}}                                                                                                                       \\
      \midrule
      Bollard         & 0.028           & 90.48             & 3.805            & 93.56               & 93.56               & 93.56               & 0.245          & 0.426           \\
      Car             & 0.033           & 92.77             & 4.044            & 93.14               & 93.14               & 93.14               & 0.544          & 0.457           \\
      Pedestrian      & 0.018           & 96.33             & 3.299            & 95.70               & 95.70               & 95.70               & 0.627          & 6.454           \\
      Pier            & 0.014           & 96.68             & 3.701            & 93.52               & 93.52               & 93.52               & 0.353          & 0.837           \\
      Plant           & 0.019           & 96.30             & 3.349            & 95.02               & 95.02               & 95.02               & 0.571          & 0.472           \\
      Safety barrier  & 0.045           & 89.59             & 3.693            & 93.87               & 93.87               & 93.87               & 0.517          & 4.070           \\
      Tire            & 0.039           & 89.52             & 3.640            & 93.27               & 93.27               & 93.27               & 0.448          & 0.100           \\
      Traffic cone    & 0.026           & 92.72             & 4.747            & 92.66               & 92.66               & 92.66               & 0.428          & 10.88           \\
      Warning sign    & 0.033           & 90.87             & 4.296            & 92.62               & 92.62               & 92.62               & 0.424          & 0.082           \\
      \midrule
      Average         & 0.028           & 92.81             & 3.864            & 93.65               & 93.65               & 93.65               & 0.462          & 2.642           \\

      \midrule \midrule
      \multicolumn{3}{l}{\textit{\textbf{\name{} (w/ iNGP)}}}                                                                                                                       \\
      \midrule
      %   Pier &  0.003 & 98.22 & 1.130 & 99.03 & 99.03 & 99.03 & 0.881 & 0.004 \\
      %   Traffic cone  & 0.002 & 100.0 & 0.770 & 99.61 & 99.61& 99.61& 0.952 &  0.060\\
      %   Tire  & 0.001 & 100.0 & 0.609 &  99.68 &  99.68 &  99.68 & 0.952 & 0.001\\
      %   Warning sign & 0.006 & 98.52 & 1.134 & 99.39 & 99.39& 99.39&  0.957 & 0.007\\
      %   Bollard  &  0.002 & 100.0 & 0.140 & 99.88& 99.88& 99.88& 0.964 & 0.003 \\
      %   Plant & 0.001 & 99.87 & 0.745 & 99.62 & 99.62& 99.62&  0.968 & 0.003\\
      %   Car &  0.005 & 99.27 & 2.241 & 97.93 & 97.93& 97.93 & 0.840 & 0.004\\
      %   Pedestrian & 0.001 & 100.0 & 1.360 & 99.28 & 99.28 & 99.28 & 0.945 & 0.025 \\
      %   Safety barrier & 0.013 & 94.31 & 2.498 & 97.00 & 97.00 & 97.00 & 0.648 & 0.019\\

      % \midrule
      % Average  & 0.004&	98.91	& 1.181 &	99.05 &	99.05&	99.05&	0.901 &	0.014\\
      Bollard         & 0.013           & 97.10             & 1.912            & 98.21               & 98.21               & 98.21               & 0.736          & 0.003           \\
      Car             & 0.014           & 97.15             & 3.417            & 94.80               & 94.80               & 94.80               & 0.627          & 0.003           \\
      Pedestrian      & 0.004           & 99.21             & 2.483            & 97.52               & 97.52               & 97.52               & 0.767          & 0.024           \\
      Pier            & 0.008           & 97.88             & 1.645            & 97.97               & 97.97               & 97.97               & 0.796          & 0.004           \\
      Plant           & 0.008           & 96.83             & 1.409            & 98.77               & 98.77               & 98.77               & 0.841          & 0.003           \\
      Safety barrier  & 0.013           & 94.31             & 2.498            & 97.00               & 97.00               & 97.00               & 0.651          & 0.019           \\
      Tire            & 0.012           & 98.10             & 1.423            & 98.40               & 98.40               & 98.40               & 0.836          & 0.001           \\
      Traffic cone    & 0.009           & 95.11             & 2.663            & 97.63               & 97.63               & 97.63               & 0.787          & 0.106           \\
      Warning sign    & 0.014           & 95.64             & 1.982            & 98.25               & 98.25               & 98.25               & 0.850          & 0.001           \\


      \midrule
      Average         & 0.011           & 96.81             & 2.159            & 97.62               & 97.62               & 97.62               & 0.766          & 0.018           \\

      \bottomrule
    \end{tabularx}
  }
  \label{tab:exp_selfdata_detail}
  \vspace{-4pt}
\end{table*}


==> latex/table/selfdata_exp_avg.tex <==
\begin{table*}[ht]
  % \footnotesize\centering\addtolength{\tabcolsep}{1.1pt}
  % \vspace{-0.2cm}
  \centering
  % \addtolength{\tabcolsep}{0.1pt}
  %  \begin{tabularx}{0.95\textwidth}{l|cccccccccc}
  \caption{\textbf{Novel LiDAR view synthesis on \datasetname{}}. Our \name{} outperforms the baseline in almost all metrics.
    % The Chamfer Distance~(C-D) in which it doesn't are biased by the density of the point clouds generated by the baseline. See \cref{fig:self-data-res} for a visual example.
    % And we find that the better C-D and F-score of the baseline are due to the fact that it generates overly dense point clouds.
  }
  \vspace{-0.2cm}
  \addtolength{\tabcolsep}{0.8pt}
  \resizebox{1\textwidth}{!}{
    \begin{tabularx}{1\textwidth}{l|cccccccc}
      \toprule
      Method                   & C-D$\downarrow$ & F-score$\uparrow$ & RMSE$\downarrow$ & $\delta$1$\uparrow$ & $\delta$2$\uparrow$ & $\delta$3$\uparrow$ & SSIM$\uparrow$ & MAE$\downarrow$ \\
      \midrule
      LiDARsim~\cite{manivasagam2020lidarsim}                                                                                                                                                \\
      PCGen~\cite{li2022pcgen} & 0.078           & 90.40             & 7.558            & 73.13               & 73.13               & 73.13               & 0.214          & 6.268           \\
      % &   0.016  & 97.35 & 8.902 &65.03 & 65.03 & 65.03 &  \\

      %  NeRF~\cite{mildenhall2021nerf}  & 0.028 & 92.81 & 3.864 & 93.65 & 93.65 & 93.65 & 0.458 & 0.010\\
      % Instance-NGP~\cite{muller2022instantNGP} \\
      \midrule
      \name{}                  & 0.004           & 98.91             & 1.181            & 99.05	99.05          & 99.05               & 0.901               & 0.014                            \\\\

      \bottomrule
    \end{tabularx}
  }
  \label{tab:exp_selfdata_avg}
  \vspace{-4pt}
\end{table*}

